Logic Haystacks: Probing LLMs Long-Context Logical Reasoning (Without Easily Identifiable Unrelated Padding)

Large language models demonstrate promising long context processing capabilities, with recent models touting context windows close to one million tokens. However, the evaluations supporting these claims often involve simple retrieval tasks or synthetic tasks padded with irrelevant text, which the models may easily detect and discard. In this work, we generate lengthy simplified English text with first-order logic representations spanning up to 2048 clauses (around 25k GPT-4 tokens). We formulate an evaluation task with evidence retrieval for contradiction detection. The long, homogeneous text is filled with distractors that are both hard to distinguish from relevant evidences and provably not interfering with them. Our evaluation of evidence retrieval shows that the effective context window is much smaller with realistic distractors, already crumbling at 128 clauses.

==> tab.tex <==

\begin{tabular}{lllllllll}
\toprule
Model size & Auxilary training & FOLIO & +ft & WANLI & +ft & CTRL & +ft & Fragments \\
\midrule
D-base & - & 49.5 & \underline{74.3} & \textbf{65.2} & \textbf{77.4} & \textbf{46.2} & \textbf{56.7} & \underline{63.6} \\
D-base & RuleTaker & 55.1 & 71.3 & 60.9 & 73.8 & 36.0 & 53.0 & 48.7 \\
D-base & LogicNLI & 50.5 & 69.3 & 61.1 & 72.4 & 38.4 & 54.4 & 56.3 \\
D-base & FLD & \underline{59.9} & 72.3 & 60.0 & 73.6 & 38.2 & 55.8 & 56.8 \\
D-base & Unigram-FOL & \textbf{64.4} & \textbf{78.2} & \underline{63.6} & \underline{75.6} & \underline{42.8} & \underline{56.6} & \textbf{65.4} \\
\midrule
D-base & $\minus$ Constrained\_Conditionals & 63.4 & 81.2 & 62.2 & 71.8 & 40.6 & 55.4 & 59.8 \\
D-base & $\minus$ Realistic\_Predicates & 62.4 & 76.2 & 65.8 & 74.4 & 41.8 & 53.2 & 68.2 \\
D-base & Unigram-LogicNLI & 57.4 & 71.3 & 61.6 & 76.4 & 38.6 & 55.6 & 57.8 \\
\midrule
D-large & - & 49.5 & 70.0 & 66.2 & 77.0 & \textbf{49.6} & \underline{62.0} & \underline{67.6} \\
D-large & RuleTaker & 58.1 & 77.2 & 68.5 & \underline{77.9} & 43.1 & 60.7 & 61.7 \\
D-large & LogicNLI & 58.7 & 73.3 & \underline{68.5} & 77.4 & 45.4 & 60.9 & 64.4 \\
D-large & FLD & \underline{60.9} & \underline{78.2} & 68.0 & 77.6 & 44.0 & 59.8 & 61.7 \\
D-large & Unigram-FOL & \textbf{63.4} & \textbf{82.2} & \textbf{75.4} & \textbf{81.6} & \underline{48.2} & \textbf{62.2} & \textbf{73.2} \\
%D-large & Unigram-FOL & 66.0 & 83.2 & 70.8 & 77.5 & 44.3 & 61.0 & 78.8 \\
\midrule
D-large & Unigram-FOL+FLD & 78.2 & 88.6 & 65.2 & 78.4 & 42.2 & 57.9 & 75.4 \\
\bottomrule
\end{tabular}

%%\begin{tabular}{lllllllll}
%\toprule
%model & training & FOLIO & FOLIO-ft & WANLI & WANLI-ft & ConTRoL & ConTRoL-ft & fragments \\
%\midrule
%D-base & - & 49.5 & \underline{74.3} & \textbf{65.2} & \textbf{77.4} & \textbf{46.2} & \textbf{56.7} & \underline{63.6} \\
%D-base & RuleTaker & 55.1 & 71.3 & 60.9 & 73.8 & 36.0 & 53.0 & 48.7 \\
%D-base & LogicNLI & 50.5 & 69.3 & 61.1 & 72.4 & 38.4 & 54.4 & 56.3 \\
%D-base & FLD & \underline{59.9} & 72.3 & 60.0 & 73.6 & 38.2 & 55.8 & 56.8 \\
%D-base & Unigram-FOL & \textbf{64.4} & \textbf{78.2} & \underline{63.6} & \underline{75.6} & \underline{42.8} & \underline{56.6} & \textbf{65.4} \\
%\midrule
%\\
%\midrule
%\\
%\vspace{1cm}
%
%D-large & - & 49.5 & 70.0 & 66.2 & 77.0 & \textbf{49.6} & \underline{62.0} & \underline{67.6} \\
%D-large & RuleTaker & 58.1 & 77.2 & 68.5 & \underline{77.9} & 43.1 & 60.7 & 61.7 \\
%D-large & LogicNLI & 58.7 & 73.3 & \underline{68.5} & 77.4 & 45.4 & 60.9 & 64.4 \\
%D-large & FLD & \underline{60.9} & \underline{78.2} & 68.0 & 77.6 & 44.0 & 59.8 & 61.7 \\
%D-large & Unigram-FOL & \textbf{63.4} & \textbf{82.2} & \textbf{75.4} & \textbf{81.6} & \underline{48.2} & \textbf{62.2} & \textbf{73.2} \\
%\midrule
%\\
%\bottomrule
%\end{tabular}
